Contextual Vision Transformers for Robust Representation Learning

We introduce Contextual Vision Transformers (ContextViT), a method designed to generate robust image representations for datasets experiencing shifts in latent factors across various groups. Derived from the concept of in-context learning, ContextViT incorporates an additional context token to encapsulate group-specific information. This integration allows the model to adjust the image representation in accordance with the group-specific context. Specifically, for a given input image, ContextViT maps images with identical group membership into this context token, which is appended to the input image tokens. Additionally, we introduce a context inference network to predict such tokens on-the-fly, given a batch of samples from the group. This enables ContextViT to adapt to new testing distributions during inference time. We demonstrate the efficacy of ContextViT across a wide range of applications. In supervised fine-tuning, we show that augmenting pre-trained ViTs with our proposed context conditioning mechanism results in consistent improvements in out-of-distribution generalization on iWildCam and FMoW. We also investigate self-supervised representation learning with ContextViT. Our experiments on the Camelyon17 pathology imaging benchmark and the JUMP-CP microscopy imaging benchmark demonstrate that ContextViT excels in learning stable image featurizations amidst distribution shift, consistently outperforming its ViT counterpart.

==> icml/experiments.tex <==


\section{Experiments}
\label{sec_main:camelyon}
In medical applications, models are often trained using data from a limited number of hospitals with the intention of deploying them across other hospitals more broadly~\cite{yala2019deep,yala2021toward,bandi2018detection}. However, this presents a challenge for the generalization of out-of-distribution data. In this section, we aim to evaluate the ability of self-supervised learning with ContextViT to achieve better out-of-distribution generalization.
\footnote{Given space constraints, we provide our ablation study and analyses in the Appendix. Additionally, we also provide evidence of the utility of ContextViT for supervised fine-tuning on iWildCam and FMoW datasets, as well as for self-supervised representation learning in microscopy imaging on the \texttt{cpg-0000} dataset.}


\paragraph{Dataset} We consider the Camelyon17-WILDS benchmark~\cite{bandi2018detection, sagawaextending}. The dataset contains 455,954 labeled and 2,999,307 unlabeled pathology images across five hospitals (3 for training, 1 for validation and 1 for testing). Given a $96\times96\times3$ image, the task is to predict whether the center region of the image contains any tumor tissue. 
\emph{We use the hospital id for context inference.}

\paragraph{Evaluation protocol}
We utilize DINO to pre-train our ViT and ContextViT models from scratch on unlabeled pathology images. Unlike previous work (\cite{sagawa2021extending}) that incorporates both in-distribution and out-of-distribution unlabeled data (Unlabeled ID\&OOD), we exclusively use images from the three training hospitals (Unlabeled ID) during pre-training stage to prevent any potential information leakage from out-of-distribution data. Given the 96 by 96 input resolution of our dataset, we opt for a smaller patch size (8 instead of 16) for the ViT models. Further details on our DINO pre-training approach can be found in the Appendix. Once pre-training is complete, we freeze the ViT parameters and train a linear classifier with SGD to predict the target label, the presence of tumors. We use the validation data for model selection and report the testing accuracy on the out-of-distribution hospitals.

\paragraph{Results}
Table~\ref{tab_main:camelyon} presents a comparison of our linear probing results (marked with$^\dagger$) with other published results on the Camelyon17 benchmark. Our DINO pre-trained ViT-S/8 baseline outperforms the much larger CLIP model in terms of linear probing (93.8 vs. 92.6), which is not surprising given the ViT-S/8 has been pre-trained on the same pathology domain. Next, we see that by conditioning our ViT-S/8 representation with other images from the same hospital within the testing batch, ContextViT-S/8 achieves an OOD accuracy of 97.5\%, significantly outperforming all baselines. Due to space constraints, we defer our ablation study and additional analyses to the appendix.
% Moreover, Figure~\ref{fig:learning_curve} demonstrates that the linear classifier built upon ContextViT-S/8 continues to enhance its OOD performance as the training of the linear classifier progresses, while the one built upon ViT-S/8 exhibits signs of over-fitting to the training data.



==> icml/introduction.tex <==
\section{Introduction}
In recent years, Vision Transformers (ViTs) have emerged as a powerful approach for image representation learning~\cite{dosovitskiyimage,khan2022transformers}. However, many real-world datasets exhibit structured variations or covariate shifts across groups, which pose challenges for standard ViT models. To address this limitation, we propose Contextual Vision Transformers (ContextViT), a novel method that leverages the notion of in-context learning~\cite{brown2020language} to produce robust feature representations for images with grouped structures, such as covariates.

ContextViT builds upon the concept of in-context learning, which was originally proposed in the domain of language processing. In-context learning involves conditioning Transformer-based models on specific contexts to enable test-time adaptation to new tasks. In our work, we extend this idea to address the challenge of \emph{covariate shift} and \emph{structured variations} in real-world datasets. Unlike traditional in-context learning approaches that condition on the whole context-dataset explicitly for each query, ContextViT infers context tokens per each group that can be shared across members of this group, such as all images collected under a shared context. A practical advantage of this modeling style is not requiring extensive memory and computing resources to serve excessive context windows.
Underlying this model is the idea of {\it mixed models}, a class of hierarchical statistical models commonly used in scientific applications, which capture fixed and random effects to represent individual- and group-level variation for observed data, but in our case those effects are latent and modeled as inferred context tokens. In-context learning is also interpreted as an implicit generative model~\cite{xie2022explanation}, but in our case the relatedness of the queries is explicitly given by the group structure, assuming a more structured style of conditioning across contexts common in real world scientific datasets collected under shared experimental conditions.

We present two variations of ContextViT: In Section~\ref{sec:cvit_oracle}, we assume contexts have been observed and infer them as parameters during training. Test-time adaptation is impractical for this model as it requires inferring a new token for a test group.
In Section~\ref{sec:cvit_context_inference}, we propose overcoming this limitation by utilizing a \emph{context inference network} to estimate these tokens on the fly given a set of examples from a group, making the model more amenable to test-time adaptation tasks.
We examine different choices for the inference network and \emph{layerwise} versus input-layer-only inference of context tokens.


We demonstrate the versatility and effectiveness of ContextViT and its variations on the challenging Camelyon17 dataset, which serves as a benchmark for distribution shift in pathology imaging. Compared to conventional ViT models, ContextViT showcases remarkable improvements in generalization, achieving significantly higher accuracy on previously unseen hospitals (97.5 compared to 93.8).

% First, we investigate the application of ContextViT for augmenting pre-trained ViTs with the extra context conditioning in a fine-tuning pass. 
% On iWildCam and FMoW, our supervised fine-tuning results consistently demonstrate substantial performance gains across three pre-trained ViT models (DINO~\cite{caron2021emerging}, SWAG~\cite{li2016revisiting} and CLIP~\cite{radford2021learning}). Beyond supervised fine-tuning, we explore the domain of self-supervised representation learning by combining DINO pre-training with ContextViT. Our findings on the microscopy imaging benchmark, \texttt{cpg-0000}, reveal that this integration enables learning of robust cell image representations that exhibit enhanced resilience to batch effects commonly encountered in microscopy imaging. 



==> icml/method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{neurips/figures/cvit.pdf}
    \vspace{-2mm}
    \caption{Contextual Vision Transformer (ContextViT). Before each Transformer layer, ContextViT applies a context inference model over all {\color{mypink}patches} (from images within the current batch that share the same group membership) to produce a {\color{myblue}context token}.
    To simplify the illustration, we present only two Transformer layers and depict a single patch embedding for each image on the left side.
 }
    \label{fig:cvit}
    \vspace{-2mm}
\end{figure*}

\section{Contextual Vision Transformer}
\label{sec:methods}

Assume $\mathcal{D}_c$ denotes a collection of samples from a distribution $P_c(\cdot)$ under potentially unknown context $c$. Our goal is as follows: given a collection of such related datasets from distributions with varying contexts $c$, we would like to learn a model that can generalize gracefully across these different domains and ideally adapt to new contexts $c^{*}$ at test time.

We assume that we observe data from multiple distributions jointly, each varying by a context $c$, so that our dataset  is comprised by their collection $\mathcal{D}=\{\mathcal{D}_1, ..., \mathcal{D}_c\}$.
We aim to learn a single shared ViT model, parameterized by $\theta$, across all sub-datasets with varying contexts.
We denote a tuple $\{x,y,c\}$ as the data describing the sample, where $x$ denotes an input, the image, and $y$ denotes an output variable such as a label or an unknown embedding, and $c$ denoting group membership for each datum to each sub-distribution $P_{c}(\cdot)$. Over the next sections we will explain our assumptions for ContextViT and will present practical implementations.

% \begin{align}
% p(Y|X, C ;\theta) = \prod_c \prod_{\{x,y\}\in \mathcal{D}_c} p(y_c|x_c, c)
% \end{align}

\subsection{In-Context Model}
\label{sec:in_context_model}
A popular paradigm for incorporating test-time conditioning in Transformers is given by in-context learning~\cite{brown2020language} and prompt-conditioning~\cite{radford2021learning,li2021prefix}.
To translate that paradigm to our task, we incorporate group membership to the representation learning task by conditioning on the members of the group, assuming the following factorization of the joint distribution over all data:

\begin{align}
\label{eq:in_context}
P(Y|X, C) = \prod_c \prod_{\{x,y\}\in \mathcal{D}_c} P(y|x, \mathcal{D}_c;\,\theta).
\end{align}

Here, we would concatenate all images belonging to context $c$ to the query image. During ViT processing, these images are patchified and represented as patch tokens, resulting in an input to the Transformer consisting of the tokens belonging to the query image and to the context images.
This process is closest to in-context reasoning as commonly applied for LLMs, but ported over to the scenario of representation learning for vision.

In practice, we can subsample patch-tokens from $\mathcal{D}_c$ up to the memory constraints and perform reasoning this way.



\subsection{Context-Token Model}

Upon further inspection, it is evident that such a process can be interpreted as performing inference over a latent variable explaining away the context-specific covariates $t_c$ as shown in the following:

\begin{align}
\label{eq:token1}
P(y|x, \mathcal{D}_c)= \int P(y|x,t_c;\,\theta) P(t_c| \mathcal{D}_c) \,\mathrm{d}t_c .
\end{align}

Here we assume an implicit hierarchical generative model of images with shared latent structure up to a contextual variable $t_c \in \mathbb{R}^{d}$ which represents an embedding of the latent covariates determining each distribution and is treated as a {\it context token}.
% Here we assume an implicit hierarchical generative model of images with shared latent structure up to a contextual variable $t_c \in \mathbb{R}^{d}$ which represents an embedding of the relevant covariates determining each distribution and is treated as a {\it context token}.
Such a context token can be characterized by its posterior distribution given the members of the group $P(t_c| \mathcal{D}_c)$ and can then be utilized in a model $P(y|x,t_c)$ to explain the impact of the contextual samples $\mathcal{D}_c$.

Under this viewpoint using Eq.\ref{eq:token1}, we can now see that the context token is shared over all members of a distribution with index $c$, allowing us to rewrite Eq.\ref{eq:in_context} such that we can break the dependence of the model on $\mathcal{D}_c$ for each data point given this context token:

\begin{align}
\label{eq:token2}
P(Y|X, C) = \prod_c \int  P(t_c| \mathcal{D}_c) \prod_{\{x,y\}\in \mathcal{D}_c} P(y|x, t_c;\,\theta) \,\mathrm{d}t_c.
\end{align}

We now have established equivalence between the in-context model, and a model which explicitly assumes existence of a context token as additional input to the forward model.
We note that recent work proposes a deeply related interpretation of in-context learning
%(bar the link to specific context distributions) 
in~\cite{xie2022explanation} supporting our view of an implicit probabilistic model.

\subsection{Oracle-Context Model}
\label{sec:cvit_oracle}
We now devise simpler formulations of the model and perform maximum likelihood inference over the context token, simplifying Eq.~\ref{eq:token2} to:

\begin{align}
\label{eq:token3}
P(Y|X, C) = \prod_c \prod_{\{x,y\}\in \mathcal{D}_c} P(y|x, t_c; \theta),
\end{align}

where $t_c$ now is a shared parameter that can be inferred per existing group during training.
We denote this model the Oracle-Context Model, since it only assumes knowledge of the indicator about which group an image belongs to, and does not require access to the other members of the group.

We can instantiate this oracle model by conditioning the ViTs with a learnable context token $t_c$ and append it to the input sequence of the Transformer: $[t_{\texttt{CLS}} , t_c, t_1 + pos_1, \ldots, t_N+pos_N]$.

The drawback is, that such a method cannot be applied during test-time outside of known distributions, since it will not be able to infer the token embedding without having seen examples from this group during training.

\subsection{Context Inference Model}
\label{sec:cvit_context_inference}
We overcome this limitation by closer matching the objective and assuming a model that performs amortized inference over the context-token parameters on the fly given $\mathcal{D}_c$ by utilizing an inference network $h(\cdot;\phi)$.


Concretely, we will again simplify $p(t_c| \mathcal{D}_c)$ to be given by maximum likelihood but this time also utilize $\mathcal{D}_c$ by posing:

\begin{align*}
\label{eq:token4}
P(Y|X, C) = \prod_c \prod_{\{x,y\}\in \mathcal{D}_c} P(y|x;\, t_c, \theta),\\
\text{with}~t_c = h(\mathcal{D}_c;\, \phi).
\end{align*}

Here, $h(\cdot;\phi)$ infers $t_c$ \emph{on the fly} when observing $\mathcal{D}_c$, and can indeed also be used during test time on a previous \emph{unknown distribution} with context $c^{*}$ time given a set of samples $\mathcal{D}_{c^{*}}$. 
There are multiple options available for instantiating the inference model $h(\cdot;\phi)$ (refer to the Appendix for more details). In the case of ContextViT (Figure~\ref{fig:cvit}), the inference model $h(\cdot;\phi)$ comprises three key components:
% We will elaborate on the choices for $t_c$, and $h(\cdot;\phi)$ in the following.

\paragraph{Mean pooling}
Given an image $x\in \mathcal{D}_c$ with its corresponding patch embeddings $t_{p_i}$, a direct way to obtain the context token $t_c$ is to aggregate the patch embeddings of all images in $\mathcal{D}_c$ through an average pooling operation
\[
t_c^{\text{mean}} = h_c^{\text{mean}}(\mathcal{D}_c) \coloneqq \frac{1}{|\mathcal{D}_c|} \sum_{x\in \mathcal{D}_c} \frac{1}{N} \sum_{x_{p_i} \in x} t_{p_i}.
\]
The input sequence for the image $x$ would then be represented as $[t_{\texttt{CLS}} , t_c^{\text{mean}}, t_1 + pos_1, \ldots, t_N+pos_N]$. In practice, instead of pooling over the entire $\mathcal{D}_{c}$, we apply mean pooling over $\mathcal{B}\cap \mathcal{D}_c$ where $\mathcal{B}$ is the current batch.

\paragraph{Linear transformation with gradients detaching}
To further enhance the context representation, we introduce a trainable linear transformation to the pooled representation. In order to prevent the patch embeddings from being penalized by the context inference model, we detach their gradients. This results in the expression 
\[h_c^{\text{linear}}(\mathcal{D}_c;\, b, W) \coloneqq b + W\cdot \texttt{detach}(t_c^{\text{mean}}).\]

\begin{table*}[t!]
    \vspace{-4mm}
    \centering
    \small
    \caption{Accuracy of linear probing of pre-trained DINO embeddings on Camelyon17-WILDS. We use $^\dagger$ to denote our implementations. Unlabeled ID\&OOD denote unlabeled pathology images from all hospitals. In our experiments, we exclude the OOD unlabeled images during the DINO pre-training stage to avoid information leak.}
    \label{tab_main:camelyon}
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{lrccccc}
        \toprule\midrule
        Backbone
        & Size
        & \begin{tabular}{@{}c@{}}Pre-training\\Method\end{tabular}
        & \begin{tabular}{@{}c@{}}Pre-training\\Dataset\end{tabular}
        & \begin{tabular}{@{}c@{}}In-distribution\\Accuracy\end{tabular}
        & \begin{tabular}{@{}c@{}}OOD\\Accuracy\end{tabular}\\\midrule
        \multicolumn{3}{l}{\emph{Fine-tuning all parameters}}\vspace{3pt}\\
        DenseNet121~\cite{koh2021wilds}        & 7.9M  & Supervised & ImageNet1K        & 90.6 & 82.0 \\
        DenseNet121~\cite{sagawa2021extending} & 7.9M  & SwaV       & Unlabeled ID\&OOD & 92.3 & 91.4 \\
        ViT-B/16~\cite{kumar2022fine}          & 86M   & DINO       & ImageNet          & ---  & 90.6 \\
        ViT-L/14~\cite{kumar2022fine}          & 303M  & CLIP       & WebImageText      & 95.2 & 96.5\\
        \midrule
        \multicolumn{3}{l}{\emph{Linear probing on frozen backbone}}\vspace{3pt}\\
        ViT-L/14~\cite{kumar2022fine}          & 303M  & CLIP       & WebImageText      & ---  & 92.6\\
        ViT-S/8$^\dagger$                      & 21.7M & DINO       & Unlabeled ID      & \textbf{98.9} & 93.8 \\
        ContextViT-S/8$^\dagger$               & 21.8M & DINO       & Unlabeled ID      & \textbf{98.9} & \textbf{97.5} \\
        \midrule\bottomrule
    \end{tabular}
\end{table*}

\paragraph{Layerwise context conditioning}
Recent work \cite{ghiasi2022vision} has shown that Transformer features progress from abstract patterns in early layers to concrete objects in later layers. We explore the application of context conditioning beyond the input layer driven by the hypothesis that patch embeddings may not be able to capture higher-level concepts. For the $l$-th Transformer layer, we use $y^{(l)}$ to denote its output and $\mathcal{D}^{(l)}_c$ to denote the collection of \emph{hidden} patch embeddings of context $c$. We propose \emph{layerwise} context conditioning which performs amortized inference over context-token parameters for each layer in the ViT instead of just propagating the input-layer token: 


\begin{align*}
    P(y^{(l)}|y^{(0)}\coloneqq x; t_c) = \prod_{l=1}^{L} P(y^{(l)} | y^{(l-1)}; t_c^{(l-1)}),\\
\text{with}~t_c^{(l)} = h(\mathcal{D}^{(l)}_c; \phi^{(l)}).
\end{align*}

For the $l$-th Transformer layer, we can express the layerwise context conditioning as
% % We apply the context inference network  from the hidden patch representations at layer $l$.
\begin{align*}
&[y_{\texttt{CLS}}^{(l)}, y_c^{(l)},  y_{p_1}^{(l)},\ldots,y_{p_N}^{(l)}]\\
&\qquad\qquad=  T^{(l)}([y_{\texttt{CLS}}^{(l-1)}, t_c^{(l-1)},  y_{p_1}^{(l-1)},\ldots,y_{p_N}^{(l-1)}]).
\end{align*}

